The improved inverted AlGaAs/GaAs interface: its relevance for high-mobility quantum wells and hybrid systems

Two dimensional electron gases (2DEGs) realized at GaAs/AlGaAs single interfaces by molecular-beam epitaxy (MBE) reach mobilities of about 15 million cm^2/Vs if the AlGaAs alloy is grown after the GaAs. Surprisingly, the mobilities may drop to a few millions for the identical but inverted AlGaAs/GaAs interface, i.e. reversed layering. Here we report on a series of inverted heterostructures with varying growth parameters including temperature, doping, and composition. Minimizing the segregation of both dopants and background impurities leads to mobilities of 13 million cm^2/Vs for inverted structures. The dependence of the mobility on electron density tunes by a gate or by illumination is found to be the identical if no doping layers exist between the 2DEG and the respective gate. Otherwise, it differs significantly compared to normal interface structures. Reducing the distance of the 2DEG to the surface down to 50nm requires an additional doping layer between 2DEG and surface in order to compensate for the surface-Schottky barrier. The suitability of such shallow inverted structures for future semiconductor-superconductor hybrid systems is discussed. Lastly, our understanding of the improved inverted interface enables us to produce optimized double-sided doped quantum wells exhibiting an electron mobility of 40 million cm^2/Vs at 1K.

==> References.tex <==
@article{sammon2018excess,
	title={Excess electron screening of remote donors and mobility in modern GaAs/AlGaAs heterostructures},
	author={Sammon, M and Chen, Tianran and Shklovskii, Boris I},
	journal={Physical Review Materials},
	volume={2},
	number={10},
	pages={104001},
	year={2018},
	publisher={APS}
}

@article{friedland1996new,
	title={New concept for the reduction of impurity scattering in remotely doped GaAs quantum wells},
	author={Friedland, K-J and Hey, R and Kostial, H and Klann, R and Ploog, K},
	journal={Physical review letters},
	volume={77},
	number={22},
	pages={4616},
	year={1996},
	publisher={APS}
}

@article{kohrbruck1990inequivalence,
	title={Inequivalence of normal and inverted interfaces of molecular-beam epitaxy grown AlGaAs/GaAs quantum wells},
	author={K{\"o}hrbr{\"u}ck, R and Munnix, S and Bimberg, D and Mars, DE and Miller, JN},
	journal={Journal of Vacuum Science \& Technology B: Microelectronics Processing and Phenomena},
	volume={8},
	number={4},
	pages={798--804},
	year={1990},
	publisher={American Vacuum Society}
}

@article{rauch1991scattering,
	title={Scattering mechanisms in inverted AlGaAs-GaAs heterostructures studied by magnetotransport measurements},
	author={Rauch, W and Gornik, E and Weimann, G and Schlapp, W},
	journal={Journal of applied physics},
	volume={70},
	number={11},
	pages={6860--6863},
	year={1991},
	publisher={American Institute of Physics}
}

@article{fischer1984improvement,
	title={Improvement of the inverted GaAs/AlGaAs heterointerface},
	author={Fischer, R and Masselink, WT and Sun, YL and Drummond, TJ and Chang, YC and Klein, MV and Morkoc, H and Anderson, E},
	journal={Journal of Vacuum Science \& Technology B: Microelectronics Processing and Phenomena},
	volume={2},
	number={2},
	pages={170--174},
	year={1984},
	publisher={American Vacuum Society}
}

@article{sajoto1989use,
	title={Use of superlattices to realize inverted GaAs/AlGaAs heterojunctions with low-temperature mobility of 2$\times$ 106 cm2/V s},
	author={Sajoto, T and Santos, M and Heremans, JJ and Shayegan, M and Heiblum, M and Weckwerth, MV and Meirav, U},
	journal={Applied physics letters},
	volume={54},
	number={9},
	pages={840--842},
	year={1989},
	publisher={American Institute of Physics}
}

@article{kane1995high,
	title={High mobility GaAs heterostructure field effect transistor for nanofabrication in which dopant-induced disorder is eliminated},
	author={Kane, BE and Pfeiffer, LN and West, KW},
	journal={Applied physics letters},
	volume={67},
	number={9},
	pages={1262--1264},
	year={1995},
	publisher={American Institute of Physics}
}

@article{akiho2021screening,
	title={Screening Effects of Superlattice Doping on the Mobility of Ga As Two-Dimensional Electron System Revealed by in situ Gate Control},
	author={Akiho, Takafumi and Muraki, Koji},
	journal={Physical Review Applied},
	volume={15},
	number={2},
	pages={024003},
	year={2021},
	publisher={APS}
}

@article{gamez2013nu,
	title={$\nu$= 5/2 fractional quantum Hall state in low-mobility electron systems: Different roles of disorder},
	author={Gamez, Gerardo and Muraki, Koji},
	journal={Physical Review B},
	volume={88},
	number={7},
	pages={075308},
	year={2013},
	publisher={APS}
}

@article{lee2019transport,
	title={Transport studies of Epi-Al/InAs two-dimensional electron gas systems for required building-blocks in topological superconductor networks},
	author={Lee, Joon Sue and Shojaei, Borzoyeh and Pendharkar, Mihir and McFadden, Anthony P and Kim, Younghyun and Suominen, Henri J and Kjaergaard, Morten and Nichele, Fabrizio and Zhang, Hao and Marcus, Charles M and others},
	journal={Nano letters},
	volume={19},
	number={5},
	pages={3083--3090},
	year={2019},
	publisher={ACS Publications}
}

@article{shabani2016two,
	title={Two-dimensional epitaxial superconductor-semiconductor heterostructures: A platform for topological superconducting networks},
	author={Shabani, Javad and Kj{\ae}rgaard, Morten and Suominen, Henri J and Kim, Younghyun and Nichele, Fabrizio and Pakrouski, Kiryl and Stankevic, T and Lutchyn, Roman M and Krogstrup, Peter and Feidenhans, R and others},
	journal={Physical Review B},
	volume={93},
	number={15},
	pages={155402},
	year={2016},
	publisher={APS}
}

@article{frolov2020topological,
	title={Topological superconductivity in hybrid devices},
	author={Frolov, SM and Manfra, MJ and Sau, JD},
	journal={Nature Physics},
	volume={16},
	number={7},
	pages={718--724},
	year={2020},
	publisher={Nature Publishing Group}
}

@article{PhysRevB.93.214504,
	author = {Zocher, Bj\"orn and Rosenow, Bernd},
	journal = {Phys. Rev. B},
	month = {Jun},
	pages = {214504},
	title = {Topological superconductivity in quantum Hall--superconductor hybrid systems},
	volume = {93},
	year = {2016}}

@article{PhysRevLett.117.096803,
	author = {Barkeshli, Maissam},
	journal = {Phys. Rev. Lett.},
	month = {Aug},
	pages = {096803},
	title = {Charge $2e/3$ Superconductivity and Topological Degeneracies without Localized Zero Modes in Bilayer Fractional Quantum Hall States},
	volume = {117},
	year = {2016}}

@article{PhysRevX.4.031009,
	author = {Vaezi, Abolhassan},
	journal = {Phys. Rev. X},
	month = {Jul},
	pages = {031009},
	title = {Superconducting Analogue of the Parafermion Fractional Quantum Hall States},
	volume = {4},
	year = {2014}}

@article{PhysRevLett.58.1260,
	author = {M\"onch, W.},
	journal = {Phys. Rev. Lett.},
	month = {Mar},
	pages = {1260--1263},
	title = {Role of virtual gap states and defects in metal-semiconductor contacts},
	volume = {58},
	year = {1987}}

@article{McLean_1988,
	author = {A B McLean and R H Williams},
	journal = {Journal of Physics C: Solid State Physics},
	month = {feb},
	number = {4},
	pages = {783--806},
	title = {Schottky contacts to cleaved {GaAs} (110) surfaces. I. Electrical properties and microscopic theories},
	volume = {21},
	year = 1988}

@article{doi:10.1063/1.94599,
	author = {Waldrop,J. R.},
	journal = {Applied Physics Letters},
	number = {10},
	pages = {1002-1004},
	title = {Schottky‐barrier height of ideal metal contacts to GaAs},
	volume = {44},
	year = {1984}}

@article{PhysRevLett.22.293,
	author = {Tsui, D. C.},
	journal = {Phys. Rev. Lett.},
	month = {Feb},
	pages = {293--295},
	title = {Observations of Surface Plasmon Excitation by Tunneling Electrons in GaAs-Pb Tunnel Junctions},
	volume = {22},
	year = {1969}}

@article{PhysRevLett.21.994,
	author = {Tsui, D. C.},
	journal = {Phys. Rev. Lett.},
	month = {Sep},
	pages = {994--996},
	title = {Evidence for Hole-To-Phonon Interaction from Tunneling Measurements in GaAs-Pb Junctions},
	volume = {21},
	year = {1968}}

@article{PhysRev.186.590,
	author = {Tsui, D. C. and Barker, A. S.},
	journal = {Phys. Rev.},
	month = {Oct},
	pages = {590--591},
	title = {Surface-Plasmon Excitation by Tunneling Electrons in GaAs-Pb Tunnel Junctions},
	volume = {186},
	year = {1969}}

@article{PhysRevLett.24.303,
	author = {Tsui, D. C.},
	journal = {Phys. Rev. Lett.},
	month = {Feb},
	pages = {303--306},
	title = {Observation of Surface Bound State and Two-Dimensional Energy Band by Electron Tunneling},
	volume = {24},
	year = {1970}}

@article{PhysRevB.4.4438,
	author = {Tsui, D. C.},
	journal = {Phys. Rev. B},
	month = {Dec},
	pages = {4438--4449},
	title = {Electron-Tunneling Studies of a Quantized Surface Accumulation Layer},
	volume = {4},
	year = {1971}}

@article{PhysRevB.14.2456,
	author = {Rowell, J. M. and Tsui, D. C.},
	journal = {Phys. Rev. B},
	month = {Sep},
	pages = {2456--2463},
	title = {Hot electron temperature in InAs measured by tunneling},
	volume = {14},
	year = {1976}}

@article{eisenstein1994compressibility,
	title={Compressibility of the two-dimensional electron gas: Measurements of the zero-field exchange energy and fractional quantum Hall gap},
	author={Eisenstein, JP and Pfeiffer, LN and West, KW},
	journal={Physical Review B},
	volume={50},
	number={3},
	pages={1760},
	year={1994},
	publisher={APS}
}

@phdthesis{scharnetzky2021ion,
	title={Ion implanted Back-gates developed for high-mobility Two-dimensional Electron systems},
	author={Scharnetzky, Jan K},
	year={2021},
	school={ETH Zurich}
}

@article{eisenstein2002insulating,
	title={Insulating and fractional quantum Hall states in the first excited Landau level},
	author={Eisenstein, JP and Cooper, KB and Pfeiffer, LN and West, KW},
	journal={Physical Review Letters},
	volume={88},
	number={7},
	pages={076801},
	year={2002},
	publisher={APS}
}

@book{tseng2011tip,
	title={Tip-based nanofabrication: Fundamentals and applications},
	author={Tseng, Ampere A},
	year={2011},
	publisher={Springer}
}

@phdthesis{simonet2017hybrid,
	title={Hybrid structures of graphene and GaAs electronic systems},
	author={Simonet, Pauline Anne Juliette},
	year={2017},
	school={ETH Zurich}
}

@article{inoue1985effects,
	title={Effects of substrate temperatures on the doping profiles of Si in selectively doped AlGaAs/GaAs/AlGaAs double-heterojunction structures},
	author={Inoue, Kaoru and Sakaki, Hiroyuki and Yoshino, Junji and Yoshioka, Yoshiaki},
	journal={Applied physics letters},
	volume={46},
	number={10},
	pages={973--975},
	year={1985},
	publisher={American Institute of Physics}
}

@article{ketterer2010compensation,
	title={Compensation mechanism in silicon-doped gallium arsenide nanowires},
	author={Ketterer, Bernt and Mikheev, Eug{\`e}ne and Uccelli, Emanuele and Fontcuberta i Morral, Anna},
	journal={Applied physics letters},
	volume={97},
	number={22},
	pages={223103},
	year={2010},
	publisher={American Institute of Physics}
}

@phdthesis{reichl2014mbe,
	title={MBE growth of ultrahigh-mobility 2DEGs in GaAs/AlGaAs},
	author={Reichl, Christian},
	year={2014},
	school={ETH Zurich}
}

@article{moison1989surface,
	title={Surface segregation of third-column atoms in group III-V arsenide compounds: Ternary alloys and heterostructures},
	author={Moison, JM and Guille, C and Houzay, F and Barthe, F and Van Rompay, M},
	journal={Physical Review B},
	volume={40},
	number={9},
	pages={6149},
	year={1989},
	publisher={APS}
}

@article{saku1994high,
	title={High-mobility inverted modulation-doped gaas/algaas heterostructures},
	author={Saku, Tadashi and Horikoshi, Yoshiji and Tarucha, Seigo},
	journal={Japanese journal of applied physics},
	volume={33},
	number={9R},
	pages={4837},
	year={1994},
	publisher={IOP Publishing}
}

@article{morkoc1982interfacial,
	title={Interfacial properties of (Al, Ga) As/GaAs structures: Effect of substrate temperature during growth by molecular beam epitaxy},
	author={Morkoc, H and Drummond, TJ and Fischer, R},
	journal={Journal of Applied Physics},
	volume={53},
	number={2},
	pages={1030--1033},
	year={1982},
	publisher={American Institute of Physics}
}

@article{sasa1984improved,
	title={Improved 2DEG Mobility in Inverted GaAs/n-AlGaAs Heterostructures Grown by MBE},
	author={Sasa, Shigehiko and Saito, Junji and Nanbu, Kazuo and Ishikawa, Tomonori and Hiyamizu, Satoshi},
	journal={Japanese journal of applied physics},
	volume={23},
	number={8A},
	pages={L573},
	year={1984},
	publisher={IOP Publishing}
}

@article{jiang1988threshold,
	title={Threshold transport of high-mobility two-dimensional electron gas in GaAs/AlGaAs heterostructures},
	author={Jiang, C and Tsui, DC and Weimann, G},
	journal={Applied physics letters},
	volume={53},
	number={16},
	pages={1533--1535},
	year={1988},
	publisher={American Institute of Physics}
}

@article{myburg1998summary,
	title={Summary of Schottky barrier height data on epitaxially grown n-and p-GaAs},
	author={Myburg, G and Auret, FD and Meyer, WE and Louw, CW and Van Staden, MJ},
	journal={Thin solid films},
	volume={325},
	number={1-2},
	pages={181--186},
	year={1998},
	publisher={Elsevier}
}

@article{reichl2015mapping,
	title={Mapping an electron wave function by a local electron scattering probe},
	author={Reichl, Christian and Dietsche, Werner and Tschirky, Thomas and Hyart, Timo and Wegscheider, Werner},
	journal={New Journal of Physics},
	volume={17},
	number={11},
	pages={113048},
	year={2015},
	publisher={IOP Publishing}
}

@article{chung2018surface,
	title={Surface segregation and the Al problem in GaAs quantum wells},
	author={Chung, Yoon Jang and Baldwin, KW and West, KW and Shayegan, M and Pfeiffer, LN},
	journal={Physical Review Materials},
	volume={2},
	number={3},
	pages={034006},
	year={2018},
	publisher={APS}
}

@article{mooney1990deep,
	title={Deep donor levels (DX centers) in III-V semiconductors},
	author={Mooney, PM},
	journal={Journal of Applied Physics},
	volume={67},
	number={3},
	pages={R1--R26},
	year={1990},
	publisher={American Institute of Physics}
}

@article{saku1996limit,
	title={Limit of electron mobility in AlGaAs/GaAs modulation-doped heterostructures},
	author={Saku, Tadashi and Horikoshi, Yoshiji and Tokura, Yasuhiro},
	journal={Japanese journal of applied physics},
	volume={35},
	number={1R},
	pages={34},
	year={1996},
	publisher={IOP Publishing}
}


@article{pfeiffer1989electron,
	title={Electron mobilities exceeding 107 cm2/V s in modulation-doped GaAs},
	author={Pfeiffer, Loren and West, KW and Stormer, HL and Baldwin, KWl},
	journal={Applied Physics Letters},
	volume={55},
	number={18},
	pages={1888--1890},
	year={1989},
	publisher={American Institute of Physics}
}


@article{gold1988scattering,
	title={Scattering time and single-particle relaxation time in a disordered two-dimensional electron gas},
	author={Gold, A},
	journal={Physical Review B},
	volume={38},
	number={15},
	pages={10798},
	year={1988},
	publisher={APS}
}


@article{umansky1997extremely,
	title={Extremely high-mobility two dimensional electron gas: Evaluation of scattering mechanisms},
	author={Umansky, V and De-Picciotto, R and Heiblum, M},
	journal={Applied physics letters},
	volume={71},
	number={5},
	pages={683--685},
	year={1997},
	publisher={American Institute of Physics}
}

@article{reuter2000increased,
	title={Increased mobility anisotropy in selectively doped Al x Ga 1- x As/GaAs heterostructures with high electron densities},
	author={Reuter, D and Versen, M and Schneider, MD and Wieck, AD},
	journal={Journal of Applied Physics},
	volume={88},
	number={1},
	pages={321--325},
	year={2000},
	publisher={American Institute of Physics}
}

@article{hwang2008limit,
	title={Limit to two-dimensional mobility in modulation-doped GaAs quantum structures: How to achieve a mobility of 100 million},
	author={Hwang, EH and Sarma, S Das},
	journal={Physical Review B},
	volume={77},
	number={23},
	pages={235437},
	year={2008},
	publisher={APS}
}


@article{pan2011impact,
	title={Impact of disorder on the 5/2 fractional quantum Hall state},
	author={Pan, W and Masuhara, N and Sullivan, NS and Baldwin, KW and West, KW and Pfeiffer, LN and Tsui, DC},
	journal={Physical review letters},
	volume={106},
	number={20},
	pages={206806},
	year={2011},
	publisher={APS}
}


@article{berl2016structured,
	title={Structured back gates for high-mobility two-dimensional electron systems using oxygen ion implantation},
	author={Berl, Matthias and Tiemann, Lars and Dietsche, Werner and Karl, Helmut and Wegscheider, Werner},
	journal={Applied Physics Letters},
	volume={108},
	number={13},
	pages={132102},
	year={2016},
	publisher={AIP Publishing LLC}
}


@article{peters2016gating,
	title={Gating versus doping: Quality parameters of two-dimensional electron systems in undoped and doped GaAs/AlGaAs heterostructures},
	author={Peters, S and Tiemann, Lars and Reichl, Christian and Wegscheider, Werner},
	journal={Physical Review B},
	volume={94},
	number={4},
	pages={045304},
	year={2016},
	publisher={APS}
}

@article{peters2017improvement,
	title={Improvement of the transport properties of a high-mobility electron system by intentional parallel conduction},
	author={Peters, Sebastian and Tiemann, Lars and Reichl, Christian and F{\"a}lt, Stefan and Dietsche, Werner and Wegscheider, Werner},
	journal={Applied Physics Letters},
	volume={110},
	number={4},
	pages={042106},
	year={2017},
	publisher={AIP Publishing LLC}
}

@article{svensson1984photoemission,
	title={Photoemission studies of the band bending on MBE-grown GaAs (001)},
	author={Svensson, SP and Kanski, J and Andersson, TG and Nilsson, P-O},
	journal={Journal of Vacuum Science \& Technology B: Microelectronics Processing and Phenomena},
	volume={2},
	number={2},
	pages={235--239},
	year={1984},
	publisher={American Vacuum Society}
}

@article{wan_induced_2015,
	title = {Induced superconductivity in high-mobility two-dimensional electron gas in gallium arsenide heterostructures},
	volume = {6},
	issn = {2041-1723},
	url = {http://www.nature.com/doifinder/10.1038/ncomms8426},
	doi = {10.1038/ncomms8426},
	pages = {7426},
	journaltitle = {Nature Communications},
	author = {Wan, Zhong and Kazakov, Aleksandr and Manfra, Michael J. and Pfeiffer, Loren N. and West, Ken W. and Rokhinson, Leonid P.},
	urldate = {2016-06-06},
	date = {2015-06-11},
	file = {ncomms8426-s1.pdf:files/6/ncomms8426-s1.pdf:application/pdf;ncomms8426.pdf:files/5/ncomms8426.pdf:application/pdf;ncomms8426.pdf:files/7/ncomms8426.pdf:application/pdf}
}

@article{eisenstein_insulating_2002,
	title = {Insulating and Fractional Quantum Hall States in the First Excited Landau Level},
	volume = {88},
	issn = {0031-9007, 1079-7114},
	url = {http://link.aps.org/doi/10.1103/PhysRevLett.88.076801},
	doi = {10.1103/PhysRevLett.88.076801},
	number = {7},
	journaltitle = {Physical Review Letters},
	author = {Eisenstein, J. P. and Cooper, K. B. and Pfeiffer, L. N. and West, K. W.},
	urldate = {2016-06-09},
	date = {2002-01-30},
	langid = {english},
	file = {PRL88_076801_2002.pdf:files/10/PRL88_076801_2002.pdf:application/pdf}
}

@article{wang_research_2016,
	title = {Research on the surface morphology of Al x Ga1−x As in molecular beam epitaxy},
	volume = {122},
	issn = {0947-8396, 1432-0630},
	url = {http://link.springer.com/10.1007/s00339-016-9720-8},
	doi = {10.1007/s00339-016-9720-8},
	number = {3},
	journaltitle = {Applied Physics A},
	author = {Wang, Yi and Wei, Wen-zhe and Yang, Chen and Guo, Xiang and Zhao, Zhen and Zhou, Hai-yue and Luo, Zi-Jang and Hu, Ming-zhe and Ding, Zhao},
	urldate = {2016-06-14},
	date = {2016-03},
	langid = {english},
	file = {art%3A10.1007%2Fs00339-016-9720-8.pdf:files/13/art%3A10.1007%2Fs00339-016-9720-8.pdf:application/pdf}
	}
	
	@article{mahalingam_gallium_1997,
		title = {Gallium desorption behavior at {AlGaAs}/{GaAs} heterointerfaces during high-temperature molecular beam epitaxy},
		volume = {15},
		issn = {0734211X},
		url = {http://scitation.aip.org/content/avs/journal/jvstb/15/4/10.1116/1.589432},
		doi = {10.1116/1.589432},
		pages = {1159},
		number = {4},
		journaltitle = {Journal of Vacuum Science \& Technology B: Microelectronics and Nanometer Structures},
		author = {Mahalingam, K.},
		urldate = {2016-06-16},
		date = {1997-07},
		file = {Gallium desorption behavior at AlGaAs_GaAs heterointerfaces durin.pdf:files/16/Gallium desorption behavior at AlGaAs_GaAs heterointerfaces durin.pdf:application/pdf}
	}
	
	@article{reithmaier_gallium_1992,
		title = {Gallium desorption during growth of (Al,Ga)As by molecular beam epitaxy},
		volume = {61},
		issn = {00036951},
		url = {http://scitation.aip.org/content/aip/journal/apl/61/10/10.1063/1.107601},
		doi = {10.1063/1.107601},
		pages = {1222},
		number = {10},
		journaltitle = {Applied Physics Letters},
		author = {Reithmaier, J.-P. and Broom, R. F. and Meier, H. P.},
		urldate = {2016-06-16},
		date = {1992},
		langid = {english},
		file = {reithmaier1992.pdf:files/18/reithmaier1992.pdf:application/pdf}
	}
	
	@article{gibson_gallium_1990,
		title = {Gallium desorption from {GaAs} and (Al,Ga)As during molecular beam epitaxy growth at high temperatures},
		volume = {57},
		issn = {00036951},
		url = {http://scitation.aip.org/content/aip/journal/apl/57/12/10.1063/1.103485},
		doi = {10.1063/1.103485},
		pages = {1203},
		number = {12},
		journaltitle = {Applied Physics Letters},
		author = {Gibson, E. M. and Foxon, C. T. and Zhang, J. and Joyce, B. A.},
		urldate = {2016-06-16},
		date = {1990},
		langid = {english},
		file = {gibson1990.pdf:files/20/gibson1990.pdf:application/pdf}
	}
	
	@article{schulte_mobility_1995,
		title = {Mobility of modulation doped {AlGaAs}/low-temperature {MBE}-grown {GaAs} heterostructures},
		volume = {24},
		issn = {0361-5235, 1543-186X},
		url = {http://link.springer.com/10.1007/BF02659699},
		doi = {10.1007/BF02659699},
		pages = {359--363},
		number = {4},
		journaltitle = {Journal of Electronic Materials},
		author = {Schulte, D. and Subramanian, S. and Ungier, L. and Bhattacharyya, K. and Arthur, J. R.},
		urldate = {2016-06-23},
		date = {1995-04},
		langid = {english},
		file = {art%3A10.1007%2FBF02659699.pdf:files/22/art%3A10.1007%2FBF02659699.pdf:application/pdf}
		}
		
		@article{marra_x-ray_1979,
			title = {X-ray total-external-reflection–Bragg diffraction: A structural study of the {GaAs}-Al interface},
			volume = {50},
			issn = {00218979},
			url = {http://scitation.aip.org/content/aip/journal/jap/50/11/10.1063/1.325845},
			doi = {10.1063/1.325845},
			shorttitle = {X-ray total-external-reflection–Bragg diffraction},
			pages = {6927},
			number = {11},
			journaltitle = {Journal of Applied Physics},
			author = {Marra, W. C.},
			urldate = {2016-06-23},
			date = {1979},
			langid = {english},
			file = {1.325845.pdf:files/24/1.325845.pdf:application/pdf}
		}
		
		@article{skeath_photoemission_1979,
			title = {Photoemission study of the interaction of Al with a {GaAs} (110) surface},
			volume = {17},
			issn = {03682048},
			url = {http://linkinghub.elsevier.com/retrieve/pii/036820487980016X},
			doi = {10.1016/0368-2048(79)80016-X},
			pages = {259--265},
			number = {4},
			journaltitle = {Journal of Electron Spectroscopy and Related Phenomena},
			author = {Skeath, Perry and Lindau, I. and Pianetta, P. and Chye, P.W. and Su, C.Y. and Spicer, W.E.},
			urldate = {2016-06-23},
			date = {1979-01},
			langid = {english},
			file = {1-s2.0-036820487980016X-main(1).pdf:files/26/1-s2.0-036820487980016X-main(1).pdf:application/pdf}
		}
		
		@article{shiraishi_ga_1992,
			title = {Ga adatom diffusion on an As-stabilized {GaAs}(001) surface via missing As dimer rows: First-principles calculation},
			volume = {60},
			issn = {00036951},
			url = {http://scitation.aip.org/content/aip/journal/apl/60/11/10.1063/1.107292},
			doi = {10.1063/1.107292},
			shorttitle = {Ga adatom diffusion on an As-stabilized {GaAs}(001) surface via missing As dimer rows},
			pages = {1363},
			number = {11},
			journaltitle = {Applied Physics Letters},
			author = {Shiraishi, Kenji},
			urldate = {2016-06-23},
			date = {1992},
			langid = {english},
			file = {1.107292.pdf:files/28/1.107292.pdf:application/pdf}
		}
		
		@article{labella_arsenic-rich_2005,
			title = {Arsenic-rich {GaAs}(0 0 1) surface structure},
			volume = {60},
			issn = {01675729},
			url = {http://linkinghub.elsevier.com/retrieve/pii/S016757290500049X},
			doi = {10.1016/j.surfrep.2005.10.001},
			pages = {1--53},
			number = {1},
			journaltitle = {Surface Science Reports},
			author = {{LaBella}, Vincent P. and Krause, Michael R. and Ding, Zhao and Thibado, Paul M.},
			urldate = {2016-06-24},
			date = {2005-12},
			langid = {english},
			file = {ssr_1.pdf:files/30/ssr_1.pdf:application/pdf}
		}
		
		@article{janes_self-assembled_2000,
			title = {Self-assembled metal/molecule/semiconductor nanostructures for electronic device and contact applications},
			volume = {29},
			issn = {0361-5235, 1543-186X},
			url = {http://link.springer.com/10.1007/s11664-000-0046-z},
			doi = {10.1007/s11664-000-0046-z},
			pages = {565--569},
			number = {5},
			journaltitle = {Journal of Electronic Materials},
			author = {Janes, D. B. and Lee, Takhee and Liu, Jia and Batistuta, M. and Chen, Nien-Po and Walsh, B. L. and Andres, R. P. and Chen, E. -H. and Melloch, M. R. and Woodall, J. M. and Reifenberger, R.},
			urldate = {2016-06-24},
			date = {2000-05},
			langid = {english},
			file = {jem_preprint.pdf:files/32/jem_preprint.pdf:application/pdf}
		}
		
		@article{melloch_low-temperature_1995,
			title = {Low-Temperature Grown {III}-V Materials},
			volume = {25},
			issn = {0084-6600, 0084-6600},
			url = {http://www.annualreviews.org/doi/abs/10.1146/annurev.ms.25.080195.002555},
			doi = {10.1146/annurev.ms.25.080195.002555},
			pages = {547--600},
			number = {1},
			journaltitle = {Annual Review of Materials Science},
			author = {Melloch, M R and Woodall, J M and Harmon, E S and Otsuka, N and Pollak, F H and Nolte, D D and Feenstra, R M and Lutz, M A},
			urldate = {2016-06-24},
			date = {1995-08},
			langid = {english},
			file = {annurev%2Ems%2E25%2E080195%2E002555(1).pdf:files/34/annurev%2Ems%2E25%2E080195%2E002555(1).pdf:application/pdf}
			}
			
			@article{whitaker_optoelectronic_1993,
				title = {Optoelectronic applications of {LTMBE} {III}–V materials},
				volume = {22},
				issn = {09215107},
				url = {http://linkinghub.elsevier.com/retrieve/pii/092151079390224B},
				doi = {10.1016/0921-5107(93)90224-B},
				pages = {61--67},
				number = {1},
				journaltitle = {Materials Science and Engineering: B},
				author = {Whitaker, John F.},
				urldate = {2016-06-24},
				date = {1993-12},
				langid = {english},
				file = {1-s2.0-092151079390224B-main.pdf:files/36/1-s2.0-092151079390224B-main.pdf:application/pdf}
			}
			
			@article{fan_molecular_2012,
				title = {Molecular beam epitaxy growth of {GaAsBi}/{GaAs}/{AlGaAs} separate confinement heterostructures},
				volume = {101},
				issn = {00036951},
				url = {http://scitation.aip.org/content/aip/journal/apl/101/18/10.1063/1.4764556},
				doi = {10.1063/1.4764556},
				pages = {181103},
				number = {18},
				journaltitle = {Applied Physics Letters},
				author = {Fan, Dongsheng and Zeng, Zhaoquan and Hu, Xian and Dorogan, Vitaliy G. and Li, Chen and Benamara, Mourad and Hawkridge, Michael E. and Mazur, Yuriy I. and Yu, Shui-Qing and Johnson, Shane R. and Wang, Zhiming M. and Salamo, Gregory J.},
				urldate = {2016-06-27},
				date = {2012},
				langid = {english},
				file = {1.4764556(1).pdf:files/38/1.4764556(1).pdf:application/pdf}
			}
			
			@article{sadeghzadeh_interfacial_2012,
				title = {Interfacial Al segregation limiting electron mobility at the inverted interface of {AlGaAs}/{GaAs} quantum well},
				volume = {27},
				issn = {0268-1242, 1361-6641},
				url = {http://stacks.iop.org/0268-1242/27/i=10/a=105009?key=crossref.a12357f5b58cf62ac6806d1facae595f},
				doi = {10.1088/0268-1242/27/10/105009},
				pages = {105009},
				number = {10},
				journaltitle = {Semiconductor Science and Technology},
				author = {Sadeghzadeh, Mohammad Ali and Azizi, Seied Mortaza},
				urldate = {2016-06-27},
				date = {2012-10-01},
				file = {sst12_10_105009(1).pdf:files/40/sst12_10_105009(1).pdf:application/pdf}
			}
			
			@article{umansky2009mbe,
				title={MBE growth of ultra-low disorder 2DEG with mobility exceeding 35$\times$ 106 cm2/V s},
				author={Umansky, V and Heiblum, M and Levinson, Y and Smet, J and N{\"u}bler, J and Dolev, M},
				journal={Journal of Crystal Growth},
				volume={311},
				number={7},
				pages={1658--1661},
				year={2009},
				publisher={Elsevier}
			}
			
			@article{hirayama_two-dimensional_1998,
				title = {Two-dimensional electron gas formed in a back-gated undoped heterostructure},
				volume = {72},
				issn = {00036951},
				url = {http://scitation.aip.org/content/aip/journal/apl/72/14/10.1063/1.121171},
				doi = {10.1063/1.121171},
				pages = {1745},
				number = {14},
				journaltitle = {Applied Physics Letters},
				author = {Hirayama, Y. and Muraki, K. and Saku, T.},
				urldate = {2016-06-28},
				date = {1998},
				langid = {english},
				file = {Two-dimensional_electron_gas_formed_in_a_back-gate(1).pdf:files/44/Two-dimensional_electron_gas_formed_in_a_back-gate(1).pdf:application/pdf}
			}
			
			@article{taneja_n-type_2016,
				title = {N-type ohmic contacts to undoped {GaAs}/{AlGaAs} quantum wells using only front-sided processing: application to ambipolar {FETs}},
				volume = {31},
				issn = {0268-1242, 1361-6641},
				url = {http://stacks.iop.org/0268-1242/31/i=6/a=065013?key=crossref.c001a5b5e6314e09fd7d6bdb2dfb3f4c},
				doi = {10.1088/0268-1242/31/6/065013},
				shorttitle = {N-type ohmic contacts to undoped {GaAs}/{AlGaAs} quantum wells using only front-sided processing},
				pages = {065013},
				number = {6},
				journaltitle = {Semiconductor Science and Technology},
				author = {Taneja, D and Sfigakis, F and Croxall, A F and Gupta, K Das and Narayan, V and Waldie, J and Farrer, I and Ritchie, D A},
				urldate = {2016-06-29},
				date = {2016-06-01},
				file = {sst_31_6_065013(1).pdf:files/46/sst_31_6_065013(1).pdf:application/pdf}
			}
			
			@article{horikoshi_photoluminescence_1987,
				title = {Photoluminescence characteristics of {AlGaAs}-{GaAs} single quantum wells grown by migration-enhanced epitaxy at 300 °C substrate temperature},
				volume = {50},
				issn = {00036951},
				url = {http://scitation.aip.org/content/aip/journal/apl/50/23/10.1063/1.97768},
				doi = {10.1063/1.97768},
				pages = {1686},
				number = {23},
				journaltitle = {Applied Physics Letters},
				author = {Horikoshi, Yoshiji and Kawashima, Minoru and Yamaguchi, Hiroshi},
				urldate = {2016-06-29},
				date = {1987},
				langid = {english},
				file = {1.97768(1).pdf:files/49/1.97768(1).pdf:application/pdf}
			}
			
			@article{tadayon_increase_1990,
				title = {Increase of electrical activation and mobility of Si-doped {GaAs}, grown at low substrate temperatures, by the migration-enhanced epitaxy method},
				volume = {67},
				issn = {00218979},
				url = {http://scitation.aip.org/content/aip/journal/jap/67/1/10.1063/1.345202},
				doi = {10.1063/1.345202},
				pages = {589},
				number = {1},
				journaltitle = {Journal of Applied Physics},
				author = {Tadayon, Bijan and Tadayon, Saied and Spencer, M. G. and Harris, G. L. and Griffin, J. and Eastman, L. F.},
				urldate = {2016-07-04},
				date = {1990},
				langid = {english},
				file = {1.345202.pdf:files/51/1.345202.pdf:application/pdf}
			}
			
			@article{currie_low-temperature_2011,
				title = {Low-temperature grown {GaAs} heterojunction metal-semiconductor-metal photodetectors improve speed and efficiency},
				volume = {99},
				issn = {00036951},
				url = {http://scitation.aip.org/content/aip/journal/apl/99/20/10.1063/1.3662392},
				doi = {10.1063/1.3662392},
				pages = {203502},
				number = {20},
				journaltitle = {Applied Physics Letters},
				author = {Currie, Marc and Quaranta, Fabio and Cola, Adriano and Gallo, Eric M. and Nabet, Bahram},
				urldate = {2016-07-07},
				date = {2011},
				langid = {english},
				file = {1.3662392(1).pdf:files/54/1.3662392(1).pdf:application/pdf}
			}
			
			@article{kawaharazuka_free_2001,
				title = {Free {GaAs} surfaces studied using a back-gated undoped {GaAs} / Al x Ga 1 − x As heterostructure},
				volume = {63},
				issn = {0163-1829, 1095-3795},
				url = {http://link.aps.org/doi/10.1103/PhysRevB.63.245309},
				doi = {10.1103/PhysRevB.63.245309},
				number = {24},
				journaltitle = {Physical Review B},
				author = {Kawaharazuka, A. and Saku, T. and Kikuchi, C. A. and Horikoshi, Y. and Hirayama, Y.},
				urldate = {2016-07-08},
				date = {2001-06-04},
				langid = {english},
				file = {kawaharazuka2001(1).pdf:files/56/kawaharazuka2001(1).pdf:application/pdf}
			}
			
			@article{pfeiffer1991si,
				title={Si dopant migration and the AlGaAs/GaAs inverted interface},
				author={Pfeiffer, Loren and Schubert, EF and West, KW and Magee, CW},
				journal={Applied physics letters},
				volume={58},
				number={20},
				pages={2258--2260},
				year={1991},
				publisher={American Institute of Physics}
			}
			
			@article{watson_impact_2015,
				title = {Impact of Heterostructure Design on Transport Properties in the Second Landau Level of \textit{In Situ} Back-Gated Two-Dimensional Electron Gases},
				volume = {3},
				issn = {2331-7019},
				url = {http://link.aps.org/doi/10.1103/PhysRevApplied.3.064004},
				doi = {10.1103/PhysRevApplied.3.064004},
				number = {6},
				journaltitle = {Physical Review Applied},
				author = {Watson, J. D. and Csáthy, G. A. and Manfra, M. J.},
				urldate = {2016-07-11},
				date = {2015-06-08},
				langid = {english},
				file = {1504.00720.pdf:files/60/1504.00720.pdf:application/pdf}
			}
			
			@article{daoudi_carbon_2014,
				title = {Carbon n-δ-doping effects on electronic and optical properties in {GaAs}/{AlGaAs} {HEMTs}},
				volume = {72},
				issn = {07496036},
				url = {http://linkinghub.elsevier.com/retrieve/pii/S074960361400130X},
				doi = {10.1016/j.spmi.2014.04.004},
				pages = {50--59},
				journaltitle = {Superlattices and Microstructures},
				author = {Daoudi, M. and Kaouach, H. and Dhifallah, I. and Ouerghi, A. and Chtourou, R.},
				urldate = {2016-07-12},
				date = {2014-08},
				langid = {english},
				file = {1-s2.0-S074960361400130X-main.pdf:files/62/1-s2.0-S074960361400130X-main.pdf:application/pdf}
			}
			
			@article{currie_low-temperature_2011-1,
				title = {Low-temperature grown {GaAs} heterojunction metal-semiconductor-metal photodetectors improve speed and efficiency},
				volume = {99},
				issn = {00036951},
				url = {http://scitation.aip.org/content/aip/journal/apl/99/20/10.1063/1.3662392},
				doi = {10.1063/1.3662392},
				pages = {203502},
				number = {20},
				journaltitle = {Applied Physics Letters},
				author = {Currie, Marc and Quaranta, Fabio and Cola, Adriano and Gallo, Eric M. and Nabet, Bahram},
				urldate = {2016-07-12},
				date = {2011},
				langid = {english},
				file = {1.3662392(2).pdf:files/64/1.3662392(2).pdf:application/pdf}
			}
			
			@article{luysberg_effects_1998,
				title = {Effects of the growth temperature and As/Ga flux ratio on the incorporation of excess As into low temperature grown {GaAs}},
				volume = {83},
				issn = {00218979},
				url = {http://scitation.aip.org/content/aip/journal/jap/83/1/10.1063/1.366723},
				doi = {10.1063/1.366723},
				pages = {561},
				number = {1},
				journaltitle = {Journal of Applied Physics},
				author = {Luysberg, M. and Sohn, H. and Prasad, A. and Specht, P. and Liliental-Weber, Z. and Weber, E. R. and Gebauer, J. and Krause-Rehberg, R.},
				urldate = {2016-07-15},
				date = {1998},
				langid = {english},
				file = {1.366723.pdf:files/67/1.366723.pdf:application/pdf}
			}
			
			@article{specht_improvement_1999,
				title = {Improvement of molecular beam epitaxy-grown low-temperature {GaAs} through p doping with Be and C},
				volume = {17},
				issn = {0734211X},
				url = {http://scitation.aip.org/content/avs/journal/jvstb/17/3/10.1116/1.590747},
				doi = {10.1116/1.590747},
				pages = {1200},
				number = {3},
				journaltitle = {Journal of Vacuum Science \& Technology B: Microelectronics and Nanometer Structures},
				author = {Specht, P. and Lutz, R. C. and Zhao, R. and Weber, E. R. and Liu, W. K. and Bacher, K. and Towner, F. J. and Stewart, T. R. and Luysberg, M.},
				urldate = {2016-07-15},
				date = {1999},
				langid = {english},
				file = {1.590747.pdf:files/69/1.590747.pdf:application/pdf}
			}
			
			@article{radomska_high_1998,
				title = {High Resistivity {AlGaAs} Grown by Low Temperature {MBE}},
				volume = {94},
				issn = {0587-4246, 1898-794X},
				url = {http://przyrbwn.icm.edu.pl/APP/PDF/94/a094z3p28.pdf},
				doi = {10.12693/APhysPolA.94.492},
				pages = {492--496},
				number = {3},
				journaltitle = {Acta Physica Polonica A},
				author = {Radomska, D. and Ratajczak, J. and Regiński, K. and Bugajski, M.},
				urldate = {2016-07-18},
				date = {1998-09},
				langid = {english},
				file = {a094z3p28.pdf:files/71/a094z3p28.pdf:application/pdf}
			}
			
			@article{yin_improved_1990,
				title = {Improved breakdown voltage in {GaAs} {MESFETs} utilizing surface layers of {GaAs} grown at a low temperature by {MBE}},
				volume = {11},
				issn = {0741-3106, 1558-0563},
				url = {http://ieeexplore.ieee.org/lpdocs/epic03/wrapper.htm?arnumber=63040},
				doi = {10.1109/55.63040},
				pages = {561--563},
				number = {12},
				journaltitle = {{IEEE} Electron Device Letters},
				author = {Yin, L.-W. and Hwang, Y. and Lee, J.H. and Kolbas, R.M. and Trew, R.J. and Mishra, U.K.},
				urldate = {2016-08-05},
				date = {1990-12},
				file = {00063040.pdf:files/74/00063040.pdf:application/pdf}
			}
			
			@article{maranowski_interface_1995,
				title = {Interface between low-temperature grown {GaAs} and undoped {GaAs} as a conduction barrier for back gates},
				volume = {66},
				issn = {00036951},
				url = {http://scitation.aip.org/content/aip/journal/apl/66/25/10.1063/1.113387},
				doi = {10.1063/1.113387},
				pages = {3459},
				number = {25},
				journaltitle = {Applied Physics Letters},
				author = {Maranowski, K. D. and Ibbetson, J. P. and Campman, K. L. and Gossard, A. C.},
				urldate = {2016-08-16},
				date = {1995},
				langid = {english},
				file = {1.113387.pdf:files/76/1.113387.pdf:application/pdf}
			}
			
			@article{huang_surface_2005,
				title = {Surface passivation of {III}-V compound semiconductors using atomic-layer-deposition-grown Al[sub 2]O[sub 3]},
				volume = {87},
				issn = {00036951},
				url = {http://scitation.aip.org/content/aip/journal/apl/87/25/10.1063/1.2146060},
				doi = {10.1063/1.2146060},
				pages = {252104},
				number = {25},
				journaltitle = {Applied Physics Letters},
				author = {Huang, M. L. and Chang, Y. C. and Chang, C. H. and Lee, Y. J. and Chang, P. and Kwo, J. and Wu, T. B. and Hong, M.},
				urldate = {2016-09-29},
				date = {2005},
				langid = {english},
				file = {10.1063@1.2146060.pdf:files/79/10.1063@1.2146060.pdf:application/pdf}
			}
			
			@article{bosund_gaas_2010,
				title = {{GaAs} surface passivation by plasma-enhanced atomic-layer-deposited aluminum nitride},
				volume = {256},
				issn = {01694332},
				url = {http://linkinghub.elsevier.com/retrieve/pii/S0169433210007762},
				doi = {10.1016/j.apsusc.2010.05.085},
				pages = {7434--7437},
				number = {24},
				journaltitle = {Applied Surface Science},
				author = {Bosund, M. and Mattila, P. and Aierken, A. and Hakkarainen, T. and Koskenvaara, H. and Sopanen, M. and Airaksinen, V.-M. and Lipsanen, H.},
				urldate = {2016-09-29},
				date = {2010-10},
				langid = {english},
				file = {1-s2.0-S0169433210007762-main.pdf:files/81/1-s2.0-S0169433210007762-main.pdf:application/pdf}
			}
			
			@article{massies_interaction_1979,
				title = {The interaction of silver and aluminium on gallium arsenide (001) surfaces: A study by mbe and associated techniques},
				volume = {80},
				issn = {00396028},
				url = {http://linkinghub.elsevier.com/retrieve/pii/0039602879907167},
				doi = {10.1016/0039-6028(79)90716-7},
				shorttitle = {The interaction of silver and aluminium on gallium arsenide (001) surfaces},
				pages = {550--556},
				journaltitle = {Surface Science},
				author = {Massies, J. and Étienne, P. and Linh, N.T.},
				urldate = {2016-09-29},
				date = {1979-02},
				langid = {english},
				file = {1-s2.0-0039602879907167-main.pdf:files/83/1-s2.0-0039602879907167-main.pdf:application/pdf}
			}
			
			@article{achtnich_secondary_1987,
				title = {Secondary ion mass spectrometry study of oxygen accumulation at {GaAs}/{AlGaAs} interfaces grown by molecular beam epitaxy},
				volume = {50},
				issn = {0003-6951, 1077-3118},
				url = {http://aip.scitation.org/doi/10.1063/1.97730},
				doi = {10.1063/1.97730},
				pages = {1730--1732},
				number = {24},
				journaltitle = {Applied Physics Letters},
				author = {Achtnich, T. and Burri, G. and Py, M. A. and Ilegems, M.},
				urldate = {2017-02-16},
				date = {1987-06-15},
				langid = {english},
				file = {1%2E97730.pdf:files/86/1%2E97730.pdf:application/pdf}
				}
				
				@article{achtnich_study_1989,
					title = {Study of oxygen incorporation in {AlGaAs} layers grown by molecular‐beam epitaxy},
					volume = {7},
					issn = {0734-2101, 1520-8559},
					url = {http://avs.scitation.org/doi/10.1116/1.575793},
					doi = {10.1116/1.575793},
					pages = {2537--2541},
					number = {4},
					journaltitle = {Journal of Vacuum Science \& Technology A: Vacuum, Surfaces, and Films},
					author = {Achtnich, T. and Burri, G. and Ilegems, M.},
					urldate = {2017-02-16},
					date = {1989-07},
					langid = {english},
					file = {1%2E575793.pdf:files/88/1%2E575793.pdf:application/pdf}
					}
					
					@article{prior_thermodynamics_1984,
						title = {The thermodynamics of oxygen incorporation into {III}–V semiconductor compounds and alloys in {MBE}},
						volume = {66},
						issn = {00220248},
						url = {http://linkinghub.elsevier.com/retrieve/pii/0022024884900769},
						doi = {10.1016/0022-0248(84)90076-9},
						pages = {55--62},
						number = {1},
						journaltitle = {Journal of Crystal Growth},
						author = {Prior, K.A. and Davies, G.J. and Heckingbottom, R.},
						urldate = {2017-02-16},
						date = {1984-01},
						langid = {english},
						file = {1-s2.0-0022024884900769-main.pdf:files/90/1-s2.0-0022024884900769-main.pdf:application/pdf}
					}
					
					@article{meynadier_optical_1985,
						title = {Optical studies of impurity trapping at the {GaAlAs}/{GaAs} interface in quantum well structures},
						volume = {58},
						issn = {0021-8979, 1089-7550},
						url = {http://aip.scitation.org/doi/10.1063/1.335516},
						doi = {10.1063/1.335516},
						pages = {4307--4312},
						number = {11},
						journaltitle = {Journal of Applied Physics},
						author = {Meynadier, M. H. and Brum, J. A. and Delalande, C. and Voos, M. and Alexandre, F. and Liévin, J. L.},
						urldate = {2017-02-16},
						date = {1985-12},
						langid = {english},
						file = {1%2E335516.pdf:files/92/1%2E335516.pdf:application/pdf}
						}
						
						@article{masselink_improved_1984,
							title = {Improved {GaAs}/{AlGaAs} single quantum wells through the use of thin superlattice buffers},
							volume = {44},
							issn = {0003-6951, 1077-3118},
							url = {http://aip.scitation.org/doi/10.1063/1.94757},
							doi = {10.1063/1.94757},
							pages = {435--437},
							number = {4},
							journaltitle = {Applied Physics Letters},
							author = {Masselink, W. T. and Klein, M. V. and Sun, Y. L. and Chang, Y. C. and Fischer, R. and Drummond, T. J. and Morkoç, H.},
							urldate = {2017-03-01},
							date = {1984-02-15},
							langid = {english},
							file = {1%2E94757.pdf:files/95/1%2E94757.pdf:application/pdf}
							}
							
							@article{sasa_improved_1984,
								title = {Improved 2DEG Mobility in Inverted {GaAs}/n-{AlGaAs} Heterostructures Grown by {MBE}},
								volume = {23},
								issn = {0021-4922},
								url = {http://stacks.iop.org/1347-4065/23/L573},
								doi = {10.1143/JJAP.23.L573},
								pages = {L573--L575},
								issue = {Part 2, No. 8},
								journaltitle = {Japanese Journal of Applied Physics},
								author = {Sasa, Shigehiko and Saito, Junji and Nanbu, Kazuo and Ishikawa, Tomonori and Hiyamizu, Satoshi},
								urldate = {2017-07-21},
								date = {1984-08-20},
								langid = {english},
								file = {Sasa_1984_Jpn._J._Appl._Phys._23_L573.pdf:files/98/Sasa_1984_Jpn._J._Appl._Phys._23_L573.pdf:application/pdf}
							}
							
							@article{maranowski_interface_1995-1,
								title = {Interface between low‐temperature grown {GaAs} and undoped {GaAs} as a conduction barrier for back gates},
								volume = {66},
								issn = {0003-6951, 1077-3118},
								url = {http://aip.scitation.org/doi/10.1063/1.113387},
								doi = {10.1063/1.113387},
								pages = {3459--3461},
								number = {25},
								journaltitle = {Applied Physics Letters},
								author = {Maranowski, K. D. and Ibbetson, J. P. and Campman, K. L. and Gossard, A. C.},
								urldate = {2017-07-26},
								date = {1995-06-19},
								langid = {english},
								file = {1%2E113387.pdf:files/101/1%2E113387.pdf:application/pdf}
								}
								
								@article{lee_fermi_1998,
									title = {The Fermi level of annealed low-temperature {GaAs} on Si-δ-doped {GaAs} grown by molecular beam epitaxy},
									volume = {83},
									issn = {0021-8979, 1089-7550},
									url = {http://aip.scitation.org/doi/10.1063/1.366719},
									doi = {10.1063/1.366719},
									pages = {486--490},
									number = {1},
									journaltitle = {Journal of Applied Physics},
									author = {Lee, W. C. and Hsu, T. M. and Wang, S. C. and Chang, M. N. and Chyi, J.-I.},
									urldate = {2017-07-27},
									date = {1998-01},
									langid = {english},
									file = {1%2E366719.pdf:files/103/1%2E366719.pdf:application/pdf}
									}
									
									@article{bennett_characteristics_1975,
										title = {Characteristics of the noradrenergic innervation of the left atrium in the chick (Gallus gallus domesticus, L.)},
										volume = {52},
										issn = {0306-4492},
										pages = {47--49},
										number = {1},
										journaltitle = {Comparative Biochemistry and Physiology. C: Comparative Pharmacology},
										shortjournal = {Comp. Biochem. Physiol. C, Comp. Pharmacol.},
										author = {Bennett, T. and Malmfors, T.},
										date = {1975-10-01},
										pmid = {202},
										keywords = {Animals, Atrial Function, Chickens, Cocaine, Heart, Heart Atria, Heart Conduction System, Myocardial Contraction, Phenoxybenzamine, Scopolamine Hydrobromide}
									}
									
									@article{moroff_yeast_1975,
										title = {Yeast glutathione reductase. Studies of the kinetics and stability of the enzyme as a function of {pH} and salt concentration},
										volume = {410},
										issn = {0006-3002},
										abstract = {1. The {pH} dependencies of the apparent Michaelis constant for oxidized glutathione and the apparent turnover number of yeast glutathione reductase ({EC} 1.6.4.2) have been determined at a fixed concentration of 0.1 {mM} {NADPH} in the range {pH} 4.5--8.0. Between {pH} 5.5 and 7.6, both of these parameters are relatively constant. The principal effect of low {pH} on the kinetics of the enzyme-catalyzed reaction is the observation of a {pH}-dependent substrate inhibition by oxidized glutathione at {pH} less than or equal 7, which is shown to correlate with the binding of oxidized glutathione to the oxidized form of the enzyme. 2. The catalytic activity of yeast glutathione reductase at {pH} 5.5 is affected by the sodium acetate buffer concentration. The stability of the oxidized and reduced forms of the enzyme at {pH} 5.5 and 25 degrees C in the absence of bovine serum albumin was studied as a function of sodium acetate concentration. The results show that activation of the catalytic activity of the enzyme at low sodium acetate concentration correlates with an effect of sodium acetate on a reduced form of the enzyme. In contrast, inhibition of the catalytic activity of the enzyme at high sodium acetate concentration correlates with an effect of sodium acetate on the oxidized form of the enzyme.},
										pages = {21--31},
										number = {1},
										journaltitle = {Biochimica Et Biophysica Acta},
										shortjournal = {Biochim. Biophys. Acta},
										author = {Moroff, G. and Brandt, K. G.},
										date = {1975-11-20},
										pmid = {74},
										keywords = {Acetates, Drug Stability, Enzyme Activation, Glutathione, Glutathione Reductase, Hydrogen-Ion Concentration, Kinetics, Osmolar Concentration, Oxidation-Reduction, Saccharomyces cerevisiae, Temperature}
									}
									
									@article{renaud_proceedings:_1975,
										title = {Proceedings: Response of identified ventromedial hypothalamic nucleus neurons to putative neurotransmitters applied by microiontophoresis},
										volume = {55},
										issn = {0007-1188},
										shorttitle = {Proceedings},
										pages = {277P--278P},
										number = {2},
										journaltitle = {British Journal of Pharmacology},
										shortjournal = {Br. J. Pharmacol.},
										author = {Renaud, L. P. and Kelly, J. S.},
										date = {1975-10},
										pmid = {115},
										pmcid = {PMC1666801},
										keywords = {Animals, Evoked Potentials, Hypothalamus, Iontophoresis, Male, Neurons, Neurotransmitter Agents, Rats}
									}
									
									@article{clegg_interrelationships_1976,
										title = {Interrelationships between water and metabolism in Artemia cysts--{II}. Carbohydrates},
										volume = {53},
										issn = {0300-9629},
										pages = {83--87},
										number = {1},
										journaltitle = {Comparative Biochemistry and Physiology. A, Comparative Physiology},
										shortjournal = {Comp Biochem Physiol A Comp Physiol},
										author = {Clegg, J. S.},
										date = {1976-01},
										pmid = {192},
										keywords = {Animals, Acclimatization, Carbohydrate Metabolism, Decapoda (Crustacea), Embryo, Nonmammalian, Glucose, Glycerol, Glycogen, Metamorphosis, Biological, Trehalose, Water}
									}
									
									@article{kavanagh_si_1993,
										title = {Si diffusion and segregation in low‐temperature grown {GaAs}},
										volume = {62},
										issn = {0003-6951, 1077-3118},
										url = {http://aip.scitation.org/doi/10.1063/1.108992},
										doi = {10.1063/1.108992},
										pages = {286--288},
										number = {3},
										journaltitle = {Applied Physics Letters},
										author = {Kavanagh, K. L. and Chang, J. C. P. and Kirchner, P. D. and Warren, A. C. and Woodall, J. M.},
										urldate = {2017-08-08},
										date = {1993-01-18},
										langid = {english},
										file = {1%2E108992.pdf:files/114/1%2E108992.pdf:application/pdf}
										}
										
										@article{newman1999upper,
											title={The upper limits of useful n-and p-type doping in GaAs and AlAs},
											author={Newman, RC},
											journal={Materials Science and Engineering: B},
											volume={66},
											number={1-3},
											pages={39--45},
											year={1999},
											publisher={Elsevier}
										}
										
										@article{jansen1990migration,
											title={Migration of Si in molecular-beam epitaxial growth of $\delta$-doped GaAs and Al0. 25Ga0. 75As},
											author={Jansen, Ph and Meuris, M and Van Rossum, Marc and Borghs, Gustaaf},
											journal={Journal of applied physics},
											volume={68},
											number={7},
											pages={3766--3768},
											year={1990},
											publisher={American Institute of Physics}
										}
										
										@article{galiev_quantum_2016,
											title = {Quantum and transport scattering times in {AlGaAs}/{InGaAs} nanoheterostructures with {AlAs} inserts in the spacer layer},
											volume = {55},
											issn = {16488504, 24243647},
											url = {http://lmaleidykla.lt/ojs/index.php/physics/article/view/3220},
											doi = {10.3952/physics.v55i4.3220},
											number = {4},
											journaltitle = {Lithuanian Journal of Physics},
											author = {Galiev, Galib B. and Vasil’evskii, Ivan S. and Klimov, Evgeniy A. and Ponomarev, Dmitry S. and Khabibullin, Rustam A. and Kulbachinskii, Vladimir A. and Gromov, Dmitry V. and Maltsev, Petr P.},
											urldate = {2017-09-08},
											date = {2016-01-11},
											file = {Lithuanian.pdf:files/121/Lithuanian.pdf:application/pdf}
										}
										
										@article{takayanagi1985superconducting,
											title={Superconducting proximity effect in the native inversion layer on InAs},
											author={Takayanagi, Hideaki and Kawakami, Tsuyoshi},
											journal={Physical review letters},
											volume={54},
											number={22},
											pages={2449},
											year={1985},
											publisher={APS}
										}
										
										@article{takayanagi1985superconducting,
											title={Superconducting proximity effect in the native inversion layer on InAs},
											author={Takayanagi, Hideaki and Kawakami, Tsuyoshi},
											journal={Physical review letters},
											volume={54},
											number={22},
											pages={2449},
											year={1985},
											publisher={APS}
										}
										
										@article{taboryski_superconductor-semiconductor-superconductor_1997,
											title = {Superconductor-semiconductor-superconductor planar junctions of aluminium on δ-doped gallium-arsenide},
											volume = {7},
											issn = {10518223},
											url = {http://ieeexplore.ieee.org/document/621821/},
											doi = {10.1109/77.621821},
											pages = {2809--2813},
											number = {2},
											journaltitle = {{IEEE} Transactions on Appiled Superconductivity},
											author = {Taboryski, R. and Clausen, T. and Kutchinsky, J. and Sorensen, C.B. and Lindelof, P.E. and Hansen, J.B. and Skov, J.L.},
											urldate = {2017-12-18},
											date = {1997-06},
											file = {Taboryski.pdf:files/129/Taboryski.pdf:application/pdf}
										}
										
										@article{takayanagi_superconducting_2002-1,
											title = {Superconducting junctions using {AlGaAs}/{GaAs} heterostructures with high Hc2 {NbN} electrodes},
											volume = {12},
											issn = {13869477},
											url = {http://linkinghub.elsevier.com/retrieve/pii/S1386947701004106},
											doi = {10.1016/S1386-9477(01)00410-6},
											pages = {922--926},
											number = {1},
											journaltitle = {Physica E: Low-dimensional Systems and Nanostructures},
											author = {Takayanagi, Hideaki and Akazaki, Tatsushi and Kawamura, Minoru and Harada, Yuichi and Nitta, Junsaku},
											urldate = {2017-12-18},
											date = {2002-01},
											langid = {english},
											file = {1-s2.0-S1386947701004106-main(1).pdf:files/131/1-s2.0-S1386947701004106-main(1).pdf:application/pdf}
										}
										
										@article{heersche2007bipolar,
											title={Bipolar supercurrent in graphene},
											author={Heersche, Hubert B and Jarillo-Herrero, Pablo and Oostinga, Jeroen B and Vandersypen, Lieven MK and Morpurgo, Alberto F},
											journal={Nature},
											volume={446},
											number={7131},
											pages={56--59},
											year={2007},
											publisher={Nature Publishing Group}
										}
										
										@article{mourik2012signatures,
											title={Signatures of Majorana fermions in hybrid superconductor-semiconductor nanowire devices},
											author={Mourik, Vincent and Zuo, Kun and Frolov, Sergey M and Plissard, SR and Bakkers, Erik PAM and Kouwenhoven, Leo P},
											journal={Science},
											volume={336},
											number={6084},
											pages={1003--1007},
											year={2012},
											publisher={American Association for the Advancement of Science}
										}
										
										@article{sacepe2011gate,
											title={Gate-tuned normal and superconducting transport at the surface of a topological insulator},
											author={Sac{\'e}p{\'e}, Benjamin and Oostinga, Jeroen B and Li, Jian and Ubaldini, Alberto and Couto, Nuno JG and Giannini, Enrico and Morpurgo, Alberto F},
											journal={Nature communications},
											volume={2},
											number={1},
											pages={1--7},
											year={2011},
											publisher={Nature Publishing Group}
										}
										
										@article{veldhorst2012josephson,
											title={Josephson supercurrent through a topological insulator surface state},
											author={Veldhorst, Menno and Snelder, Marieke and Hoek, Marcel and Gang, Tian and Guduru, VK and Wang, XL and Zeitler, Uli and van der Wiel, Wilfred Gerard and Golubov, AA and Hilgenkamp, Hans and others},
											journal={Nature materials},
											volume={11},
											number={5},
											pages={417--421},
											year={2012},
											publisher={Nature Publishing Group}
										}
										
										@article{sato2016majorana,
											title={Majorana fermions and topology in superconductors},
											author={Sato, Masatoshi and Fujimoto, Satoshi},
											journal={Journal of the Physical Society of Japan},
											volume={85},
											number={7},
											pages={072001},
											year={2016},
											publisher={The Physical Society of Japan}
										}
										
										@article{saku1998high,
											title={High-mobility two-dimensional electron gas in an undoped heterostructure: Mobility enhancement after illumination},
											author={Saku, Tadashi and Muraki, Koji and Hirayama, Yoshiro},
											journal={Japanese journal of applied physics},
											volume={37},
											number={7A},
											pages={L765},
											year={1998},
											publisher={IOP Publishing}
										}
										
										
										
										@article{gurvitch_ohmic_1986,
											title = {Ohmic, superconducting, shallow {AuGe}/Nb contacts to {GaAs}},
											volume = {60},
											issn = {0021-8979, 1089-7550},
											url = {http://aip.scitation.org/doi/10.1063/1.337738},
											doi = {10.1063/1.337738},
											pages = {3204--3210},
											number = {9},
											journaltitle = {Journal of Applied Physics},
											author = {Gurvitch, M. and Kastalsky, A. and Schwarz, S. and Hwang, D. M. and Butherus, D. and Pearton, S. and Gardner, C. R.},
											urldate = {2018-02-27},
											date = {1986-11},
											langid = {english},
											file = {1.337738.pdf:files/150/1.337738.pdf:application/pdf}
										}
										
										@article{lenssen_superconducting_1993,
											title = {Superconducting contacts to a two-dimensional electron gas in {GaAs}/{AlGaAs}-heterostructures},
											volume = {3},
											issn = {1051-8223, 1558-2515},
											url = {http://ieeexplore.ieee.org/document/233575/},
											doi = {10.1109/77.233575},
											pages = {1961--1963},
											number = {1},
											journaltitle = {{IEEE} Transactions on Applied Superconductivity},
											author = {Lenssen, K.-M.H. and Matters, M. and Harmans, C.J.P.M. and Mooij, J.E. and Leys, M.R. and van der Vleuten, W. and Wolter, J.H.},
											urldate = {2018-06-08},
											date = {1993-03},
											file = {Lenssen et al. - 1993 - Superconducting contacts to a two-dimensional elec.pdf:files/153/Lenssen et al. - 1993 - Superconducting contacts to a two-dimensional elec.pdf:application/pdf}
										}
										
										@article{taboryski_superconductor-semiconductor-superconductor_1997-1,
											title = {Superconductor-semiconductor-superconductor planar junctions of aluminium on δ-doped gallium-arsenide},
											volume = {7},
											issn = {10518223},
											url = {http://ieeexplore.ieee.org/document/621821/},
											doi = {10.1109/77.621821},
											pages = {2809--2813},
											number = {2},
											journaltitle = {{IEEE} Transactions on Appiled Superconductivity},
											author = {Taboryski, R. and Clausen, T. and Kutchinsky, J. and Sorensen, C.B. and Lindelof, P.E. and Hansen, J.B. and Skov, J.L.},
											urldate = {2018-06-08},
											date = {1997-06},
											file = {Taboryski et al. - 1997 - Superconductor-semiconductor-superconductor planar.pdf:files/155/Taboryski et al. - 1997 - Superconductor-semiconductor-superconductor planar.pdf:application/pdf}
										}
										
										@article{wan2015induced,
											title={Induced superconductivity in high-mobility two-dimensional electron gas in gallium arsenide heterostructures},
											author={Wan, Zhong and Kazakov, Aleksandr and Manfra, Michael J and Pfeiffer, Loren N and West, Ken W and Rokhinson, Leonid P},
											journal={Nature communications},
											volume={6},
											number={1},
											pages={1--5},
											year={2015},
											publisher={Nature Publishing Group}
										}
										
										@inproceedings{lei_oscillations_2010,
											location = {Hong Kong, China},
											title = {Oscillations of nonlinear magnetoresistance in microwave-irradiated 2D semiconductors},
											isbn = {978-1-4244-3543-2},
											url = {http://ieeexplore.ieee.org/document/5424468/},
											doi = {10.1109/INEC.2010.5424468},
											eventtitle = {2010 {IEEE} 3rd International Nanoelectronics Conference ({INEC})},
											pages = {16--17},
											booktitle = {2010 3rd International Nanoelectronics Conference ({INEC})},
											publisher = {{IEEE}},
											author = {Lei, X. L.},
											urldate = {2018-08-28},
											date = {2010-01},
											file = {Lei - 2010 - Oscillations of nonlinear magnetoresistance in mic.pdf:files/161/Lei - 2010 - Oscillations of nonlinear magnetoresistance in mic.pdf:application/pdf}
										}
										
										@article{wu_formation_2018,
											title = {Formation of helical domain walls in the fractional quantum Hall regime as a step toward realization of high-order non-Abelian excitations},
											volume = {97},
											issn = {2469-9950, 2469-9969},
											url = {https://link.aps.org/doi/10.1103/PhysRevB.97.245304},
											doi = {10.1103/PhysRevB.97.245304},
											number = {24},
											journaltitle = {Physical Review B},
											author = {Wu, Tailung and Wan, Zhong and Kazakov, Aleksandr and Wang, Ying and Simion, George and Liang, Jingcheng and West, Kenneth W. and Baldwin, Kirk and Pfeiffer, Loren N. and Lyanda-Geller, Yuli and Rokhinson, Leonid P.},
											urldate = {2018-08-28},
											date = {2018-06-07},
											langid = {english},
											file = {Wu et al. - 2018 - Formation of helical domain walls in the fractiona.pdf:files/164/Wu et al. - 2018 - Formation of helical domain walls in the fractiona.pdf:application/pdf}
										}
										
										@article{wu_formation_2018-1,
											title = {Formation of helical domain walls in the fractional quantum Hall regime as a step toward realization of high-order non-Abelian excitations},
											volume = {97},
											issn = {2469-9950, 2469-9969},
											url = {https://link.aps.org/doi/10.1103/PhysRevB.97.245304},
											doi = {10.1103/PhysRevB.97.245304},
											number = {24},
											journaltitle = {Physical Review B},
											author = {Wu, Tailung and Wan, Zhong and Kazakov, Aleksandr and Wang, Ying and Simion, George and Liang, Jingcheng and West, Kenneth W. and Baldwin, Kirk and Pfeiffer, Loren N. and Lyanda-Geller, Yuli and Rokhinson, Leonid P.},
											urldate = {2018-08-28},
											date = {2018-06-07},
											langid = {english}
										}
										
										@article{bouscher_andreev_2018,
											title = {Andreev reflection enhancement in semiconductor-superconductor structures},
											volume = {97},
											issn = {2469-9950, 2469-9969},
											url = {https://link.aps.org/doi/10.1103/PhysRevB.97.054512},
											doi = {10.1103/PhysRevB.97.054512},
											number = {5},
											journaltitle = {Physical Review B},
											author = {Bouscher, Shlomi and Winik, Roni and Hayat, Alex},
											urldate = {2018-09-24},
											date = {2018-02-20},
											langid = {english},
											file = {Bouscher et al. - 2018 - Andreev reflection enhancement in semiconductor-su.pdf:files/168/Bouscher et al. - 2018 - Andreev reflection enhancement in semiconductor-su.pdf:application/pdf}
										}
										
										@article{chevallier_donor_1985,
											title = {Donor neutralization in {GaAs}(Si) by atomic hydrogen},
											volume = {47},
											issn = {0003-6951, 1077-3118},
											url = {http://aip.scitation.org/doi/10.1063/1.96284},
											doi = {10.1063/1.96284},
											pages = {108--110},
											number = {2},
											journaltitle = {Applied Physics Letters},
											author = {Chevallier, J. and Dautremont‐Smith, W. C. and Tu, C. W. and Pearton, S. J.},
											urldate = {2018-10-10},
											date = {1985-07-15},
											langid = {english},
											file = {Chevallier et al. - 1985 - Donor neutralization in GaAs(Si) by atomic hydroge.pdf:files/171/Chevallier et al. - 1985 - Donor neutralization in GaAs(Si) by atomic hydroge.pdf:application/pdf}
										}
										
										@article{clarke_exotic_2013,
											title = {Exotic non-Abelian anyons from conventional fractional quantum Hall states},
											volume = {4},
											issn = {2041-1723},
											url = {http://www.nature.com/articles/ncomms2340},
											doi = {10.1038/ncomms2340},
											number = {1},
											journaltitle = {Nature Communications},
											author = {Clarke, David J. and Alicea, Jason and Shtengel, Kirill},
											urldate = {2018-11-08},
											date = {2013-12},
											langid = {english},
											file = {1.96284(1).pdf:files/175/1.96284(1).pdf:application/pdf;Volltext:files/174/Clarke et al. - 2013 - Exotic non-Abelian anyons from conventional fracti.pdf:application/pdf}
										}
										
										@article{vaezi_fractional_2013,
											title = {Fractional topological superconductor with fractionalized Majorana fermions},
											volume = {87},
											issn = {1098-0121, 1550-235X},
											url = {https://link.aps.org/doi/10.1103/PhysRevB.87.035132},
											doi = {10.1103/PhysRevB.87.035132},
											number = {3},
											journaltitle = {Physical Review B},
											author = {Vaezi, Abolhassan},
											urldate = {2019-01-16},
											date = {2013-01-25},
											langid = {english},
											file = {Eingereichte Version:files/178/Vaezi - 2013 - Fractional topological superconductor with fractio.pdf:application/pdf;PhysRevB.87.035132.pdf:files/179/PhysRevB.87.035132.pdf:application/pdf}
										}
										
										
										
										@article{braun1994situ,
											title={In situ technique for measuring Ga segregation and interface roughness at GaAs/AlGaAs interfaces},
											author={Braun, W and Ploog, KH},
											journal={Journal of applied physics},
											volume={75},
											number={4},
											pages={1993--2001},
											year={1994},
											publisher={American Institute of Physics}
										}
										
										@article{singh_theoretical_1984,
											title = {Theoretical investigations of the nature of the normal and inverted {GaAs}–{AlGaAs} structures grown by molecular beam epitaxy},
											volume = {2},
											issn = {0734211X},
											url = {http://scitation.aip.org/content/avs/journal/jvstb/2/3/10.1116/1.582841},
											doi = {10.1116/1.582841},
											pages = {576},
											number = {3},
											journaltitle = {Journal of Vacuum Science \& Technology B: Microelectronics and Nanometer Structures},
											author = {Singh, Jasprit},
											urldate = {2019-06-21},
											date = {1984},
											langid = {english},
											file = {Singh - 1984 - Theoretical investigations of the nature of the no.pdf:files/184/Singh - 1984 - Theoretical investigations of the nature of the no.pdf:application/pdf}
										}
										
										@article{cisneros-de-la-rosa_effect_2014,
											title = {Effect of surface states on the electrical properties of {MBE} grown modulation doped {AlGaAs}/{GaAs}},
											volume = {32},
											issn = {2166-2746, 2166-2754},
											url = {http://avs.scitation.org/doi/10.1116/1.4863677},
											doi = {10.1116/1.4863677},
											pages = {02C110},
											number = {2},
											journaltitle = {Journal of Vacuum Science \& Technology B, Nanotechnology and Microelectronics: Materials, Processing, Measurement, and Phenomena},
											author = {Cisneros-de-la-Rosa, Alejandro and Cortes-Mestizo, Irving Eduardo and Cruz-Hernández, Esteban and Méndez-García, Víctor Hugo and Zamora-Peredo, Luis and González-Fernández, José Vulfrano and Balderas-Navarro, Raúl and Gorbatchev, Andrei Yu. and López-López, Máximo},
											urldate = {2019-06-26},
											date = {2014-03},
											langid = {english},
											file = {Cisneros-de-la-Rosa et al. - 2014 - Effect of surface states on the electrical propert.pdf:files/187/Cisneros-de-la-Rosa et al. - 2014 - Effect of surface states on the electrical propert.pdf:application/pdf}
										}
										
										@article{shang_effects_2004,
											title = {Effects of indium doping on the properties of {AlAs}/{GaAs} quantum wells and inverted {AlGaAs}/{GaAs} two-dimensional electron gas},
											volume = {19},
											issn = {0268-1242, 1361-6641},
											url = {http://stacks.iop.org/0268-1242/19/i=3/a=042?key=crossref.4212ff37fe615e0ac0b473406c3f509f},
											doi = {10.1088/0268-1242/19/3/042},
											pages = {519--522},
											number = {3},
											journaltitle = {Semiconductor Science and Technology},
											author = {Shang, X Z and Wang, W C and Wu, S D and Xing, Z G and Guo, L W and Wang, W X and Huang, Q and Zhou, J M},
											urldate = {2019-07-12},
											date = {2004-03-01},
											file = {Shang et al. - 2004 - Effects of indium doping on the properties of AlAs.pdf:files/190/Shang et al. - 2004 - Effects of indium doping on the properties of AlAs.pdf:application/pdf}
										}
										
										@article{mak_distinguishing_2010,
											title = {Distinguishing impurity concentrations in {GaAs} and {AlGaAs} using very shallow undoped heterostructures},
											volume = {97},
											issn = {0003-6951, 1077-3118},
											url = {http://aip.scitation.org/doi/10.1063/1.3522651},
											doi = {10.1063/1.3522651},
											pages = {242107},
											number = {24},
											journaltitle = {Applied Physics Letters},
											author = {Mak, W. Y. and Das Gupta, K. and Beere, H. E. and Farrer, I. and Sfigakis, F. and Ritchie, D. A.},
											urldate = {2019-07-12},
											date = {2010-12-13},
											langid = {english},
											file = {Eingereichte Version:files/192/Mak et al. - 2010 - Distinguishing impurity concentrations in GaAs and.pdf:application/pdf}
										}
										
										@article{kawaharazuka_formation_2000,
											title = {Formation of a two-dimensional electron gas in an inverted undoped heterostructure with a shallow channel depth},
											volume = {87},
											issn = {0021-8979, 1089-7550},
											url = {http://aip.scitation.org/doi/10.1063/1.371965},
											doi = {10.1063/1.371965},
											pages = {952--954},
											number = {2},
											journaltitle = {Journal of Applied Physics},
											author = {Kawaharazuka, A. and Saku, T. and Hirayama, Y. and Horikoshi, Y.},
											urldate = {2019-07-12},
											date = {2000-01-15},
											langid = {english},
											file = {Kawaharazuka et al. - 2000 - Formation of a two-dimensional electron gas in an .pdf:files/194/Kawaharazuka et al. - 2000 - Formation of a two-dimensional electron gas in an .pdf:application/pdf}
										}
										
										@article{saku_high-mobility_1998-2,
											title = {High-Mobility Two-Dimensional Electron Gas in an Undoped Heterostructure: Mobility Enhancement after Illumination},
											volume = {37},
											issn = {00214922},
											url = {http://stacks.iop.org/1347-4065/37/L765},
											doi = {10.1143/JJAP.37.L765},
											shorttitle = {High-Mobility Two-Dimensional Electron Gas in an Undoped Heterostructure},
											pages = {L765--L767},
											issue = {Part 2, No. 7A},
											journaltitle = {Japanese Journal of Applied Physics},
											author = {Saku, Tadashi and Muraki, Koji and Hirayama, Yoshiro},
											urldate = {2019-07-16},
											date = {1998-07-01},
											file = {Saku et al. - 1998 - High-Mobility Two-Dimensional Electron Gas in an U.pdf:files/198/Saku et al. - 1998 - High-Mobility Two-Dimensional Electron Gas in an U.pdf:application/pdf;Tadashi Saku_1998_Jpn._J._Appl._Phys._37_L765(2).pdf:files/199/Tadashi Saku_1998_Jpn._J._Appl._Phys._37_L765(2).pdf:application/pdf;Tadashi Saku_1998_Jpn._J._Appl._Phys._37_L765(3).pdf:files/221/Tadashi Saku_1998_Jpn._J._Appl._Phys._37_L765(3).pdf:application/pdf;Tadashi Saku_1998_Jpn._J._Appl._Phys._37_L765(4).pdf:files/240/Tadashi Saku_1998_Jpn._J._Appl._Phys._37_L765(4).pdf:application/pdf}
										}
										
										@article{hirayama_two-dimensional_1998-1,
											title = {Two-dimensional electron gas formed in a back-gated undoped heterostructure},
											volume = {72},
											issn = {0003-6951, 1077-3118},
											url = {http://aip.scitation.org/doi/10.1063/1.121171},
											doi = {10.1063/1.121171},
											pages = {1745--1747},
											number = {14},
											journaltitle = {Applied Physics Letters},
											author = {Hirayama, Y. and Muraki, K. and Saku, T.},
											urldate = {2020-01-21},
											date = {1998-04-06},
											langid = {english}
										}
										
										@article{horvath_near-interface_1990,
											title = {Near-interface concentration reduction in n-type Au/Cr{GaAs} Schottky contacts},
											volume = {40},
											issn = {0042207X},
											url = {https://linkinghub.elsevier.com/retrieve/pii/0042207X9090156S},
											doi = {10.1016/0042-207X(90)90156-S},
											pages = {201--203},
											number = {1},
											journaltitle = {Vacuum},
											author = {Horváth, {ZsJ} and Gyúró, I and Németh-Sallay, M and Tüttö, P},
											urldate = {2020-02-14},
											date = {1990-01},
											langid = {english},
											file = {Horváth et al. - 1990 - Near-interface concentration reduction in n-type A.pdf:files/202/Horváth et al. - 1990 - Near-interface concentration reduction in n-type A.pdf:application/pdf}
										}
										
										@article{schmidt_chemically_1989,
											title = {Chemically modified {GaAs} Schottky barrier variation},
											volume = {7},
											issn = {0734211X},
											url = {http://scitation.aip.org/content/avs/journal/jvstb/7/4/10.1116/1.584590},
											doi = {10.1116/1.584590},
											pages = {980},
											number = {4},
											journaltitle = {Journal of Vacuum Science \& Technology B: Microelectronics and Nanometer Structures},
											author = {Schmidt, M. T.},
											urldate = {2020-02-14},
											date = {1989-07},
											file = {Schmidt - 1989 - Chemically modified GaAs Schottky barrier variatio.pdf:files/204/Schmidt - 1989 - Chemically modified GaAs Schottky barrier variatio.pdf:application/pdf}
										}
										
										@article{chand_growth_1993,
											title = {Growth of high quality {AlGaAs}/{GaAs} heterostructures by molecular beam epitaxy for photonic and electronic device applications},
											volume = {231},
											issn = {00406090},
											url = {https://linkinghub.elsevier.com/retrieve/pii/004060909390709X},
											doi = {10.1016/0040-6090(93)90709-X},
											pages = {143--157},
											number = {1},
											journaltitle = {Thin Solid Films},
											author = {Chand, Naresh},
											urldate = {2020-03-22},
											date = {1993-08},
											langid = {english},
											file = {Chand - 1993 - Growth of high quality AlGaAsGaAs heterostructure.pdf:files/206/Chand - 1993 - Growth of high quality AlGaAsGaAs heterostructure.pdf:application/pdf}
										}
										
										@article{schubert_fermi-level-pinning-induced_1990,
											title = {Fermi-level-pinning-induced impurity redistribution in semiconductors during epitaxial growth},
											volume = {42},
											issn = {0163-1829, 1095-3795},
											url = {https://link.aps.org/doi/10.1103/PhysRevB.42.1364},
											doi = {10.1103/PhysRevB.42.1364},
											pages = {1364--1368},
											number = {2},
											journaltitle = {Physical Review B},
											author = {Schubert, E. F. and Kuo, J. M. and Kopf, R. F. and Jordan, A. S. and Luftman, H. S. and Hopkins, L. C.},
											urldate = {2020-03-22},
											date = {1990-07-15},
											langid = {english},
											file = {Schubert et al. - 1990 - Fermi-level-pinning-induced impurity redistributio.pdf:files/208/Schubert et al. - 1990 - Fermi-level-pinning-induced impurity redistributio.pdf:application/pdf}
										}
										
										@article{morkoc1982interfacial,
											title={Interfacial properties of (Al, Ga) As/GaAs structures: Effect of substrate temperature during growth by molecular beam epitaxy},
											author={Morkoc, H and Drummond, TJ and Fischer, R},
											journal={Journal of Applied Physics},
											volume={53},
											number={2},
											pages={1030--1033},
											year={1982},
											publisher={American Institute of Physics}
										}
										
										@article{gardner_modified_2016,
											title = {Modified {MBE} hardware and techniques and role of gallium purity for attainment of two dimensional electron gas mobility {\textgreater}35×106cm2/V s in {AlGaAs}/{GaAs} quantum wells grown by {MBE}},
											volume = {441},
											issn = {00220248},
											url = {https://linkinghub.elsevier.com/retrieve/pii/S0022024816300367},
											doi = {10.1016/j.jcrysgro.2016.02.010},
											pages = {71--77},
											journaltitle = {Journal of Crystal Growth},
											author = {Gardner, Geoffrey C. and Fallahi, Saeed and Watson, John D. and Manfra, Michael J.},
											urldate = {2020-03-30},
											date = {2016-05},
											langid = {english},
											file = {Akzeptierte Version:files/212/Gardner et al. - 2016 - Modified MBE hardware and techniques and role of g.pdf:application/pdf;MBEpaperpublished.pdf:files/213/MBEpaperpublished.pdf:application/pdf}
										}
										
										@article{cisneros-de-la-rosa_effect_2014-1,
											title = {Effect of surface states on the electrical properties of {MBE} grown modulation doped {AlGaAs}/{GaAs}},
											volume = {32},
											issn = {2166-2746, 2166-2754},
											url = {http://avs.scitation.org/doi/10.1116/1.4863677},
											doi = {10.1116/1.4863677},
											pages = {02C110},
											number = {2},
											journaltitle = {Journal of Vacuum Science \& Technology B, Nanotechnology and Microelectronics: Materials, Processing, Measurement, and Phenomena},
											author = {Cisneros-de-la-Rosa, Alejandro and Cortes-Mestizo, Irving Eduardo and Cruz-Hernández, Esteban and Méndez-García, Víctor Hugo and Zamora-Peredo, Luis and González-Fernández, José Vulfrano and Balderas-Navarro, Raúl and Gorbatchev, Andrei Yu. and López-López, Máximo},
											urldate = {2020-04-05},
											date = {2014-03},
											langid = {english},
											file = {Cisneros-de-la-Rosa et al. - 2014 - Effect of surface states on the electrical propert.pdf:files/215/Cisneros-de-la-Rosa et al. - 2014 - Effect of surface states on the electrical propert.pdf:application/pdf}
										}
										
										@article{manfra_molecular_2014,
											title = {Molecular Beam Epitaxy of Ultra-High-Quality {AlGaAs}/{GaAs} Heterostructures: Enabling Physics in Low-Dimensional Electronic Systems},
											volume = {5},
											issn = {1947-5454, 1947-5462},
											url = {http://www.annualreviews.org/doi/10.1146/annurev-conmatphys-031113-133905},
											doi = {10.1146/annurev-conmatphys-031113-133905},
											shorttitle = {Molecular Beam Epitaxy of Ultra-High-Quality {AlGaAs}/{GaAs} Heterostructures},
											pages = {347--373},
											number = {1},
											journaltitle = {Annual Review of Condensed Matter Physics},
											author = {Manfra, Michael J.},
											urldate = {2020-04-05},
											date = {2014-03},
											langid = {english},
											file = {annurev-conmatphys-031113-133905.pdf:files/218/annurev-conmatphys-031113-133905.pdf:application/pdf;Eingereichte Version:files/217/Manfra - 2014 - Molecular Beam Epitaxy of Ultra-High-Quality AlGaA.pdf:application/pdf}
										}
										
										@article{mak_distinguishing_2010-1,
											title = {Distinguishing impurity concentrations in {GaAs} and {AlGaAs} using very shallow undoped heterostructures},
											volume = {97},
											issn = {0003-6951, 1077-3118},
											url = {http://aip.scitation.org/doi/10.1063/1.3522651},
											doi = {10.1063/1.3522651},
											pages = {242107},
											number = {24},
											journaltitle = {Applied Physics Letters},
											author = {Mak, W. Y. and Das Gupta, K. and Beere, H. E. and Farrer, I. and Sfigakis, F. and Ritchie, D. A.},
											urldate = {2020-04-05},
											date = {2010-12-13},
											langid = {english},
											file = {Eingereichte Version:files/220/Mak et al. - 2010 - Distinguishing impurity concentrations in GaAs and.pdf:application/pdf}
										}
										
										@article{silberman_fermi_1991,
											title = {Fermi level pinning at epitaxial Si on {GaAs}(100) interfaces},
											volume = {59},
											issn = {0003-6951, 1077-3118},
											url = {http://aip.scitation.org/doi/10.1063/1.105712},
											doi = {10.1063/1.105712},
											pages = {3300--3302},
											number = {25},
											journaltitle = {Applied Physics Letters},
											author = {Silberman, J. A. and de Lyon, T. J. and Woodall, J. M.},
											urldate = {2020-04-13},
											date = {1991-12-16},
											langid = {english},
											file = {Silberman et al. - 1991 - Fermi level pinning at epitaxial Si on GaAs(100) i.pdf:files/223/Silberman et al. - 1991 - Fermi level pinning at epitaxial Si on GaAs(100) i.pdf:application/pdf}
										}
										
										@article{hwang_limit_2008,
											title = {Limit to two-dimensional mobility in modulation-doped {GaAs} quantum structures: How to achieve a mobility of 100 million},
											volume = {77},
											issn = {1098-0121, 1550-235X},
											url = {https://link.aps.org/doi/10.1103/PhysRevB.77.235437},
											doi = {10.1103/PhysRevB.77.235437},
											shorttitle = {Limit to two-dimensional mobility in modulation-doped {GaAs} quantum structures},
											number = {23},
											journaltitle = {Physical Review B},
											author = {Hwang, E. H. and Das Sarma, S.},
											urldate = {2020-04-14},
											date = {2008-06-25},
											langid = {english},
											file = {0804.4684.pdf:files/226/0804.4684.pdf:application/pdf;Eingereichte Version:files/225/Hwang und Das Sarma - 2008 - Limit to two-dimensional mobility in modulation-do.pdf:application/pdf}
										}
										
										@article{buchner_optical_2017,
											title = {Optical investigation of electrical spin injection into an inverted two-dimensional electron gas structure},
											volume = {95},
											issn = {2469-9950, 2469-9969},
											url = {https://link.aps.org/doi/10.1103/PhysRevB.95.035304},
											doi = {10.1103/PhysRevB.95.035304},
											number = {3},
											journaltitle = {Physical Review B},
											author = {Buchner, M. and Kuczmik, T. and Oltscher, M. and Ciorga, M. and Korn, T. and Loher, J. and Schuh, D. and Schüller, C. and Bougeard, D. and Weiss, D. and Back, C. H.},
											urldate = {2020-04-15},
											date = {2017-01-13},
											langid = {english},
											file = {Eingereichte Version:files/228/Buchner et al. - 2017 - Optical investigation of electrical spin injection.pdf:application/pdf;PhysRevB.95.035304.pdf:files/229/PhysRevB.95.035304.pdf:application/pdf}
										}
										
										@article{gonzalez1986silicon,
											title={Silicon migration during MBE growth of doped (A1, Ga) As films},
											author={Gonzalez, Luisa and Clegg, JB and Hilton, D and Gowers, JP and Foxon, CT and Joyce, BA},
											journal={Applied Physics A},
											volume={41},
											number={3},
											pages={237--241},
											year={1986},
											publisher={Springer}
										}
										
										
										@article{baba1986elimination,
											title={Elimination of a DX-center by an AlAs/n-GaAs superlattice and its application to 2DEGFETs},
											author={Baba, Toshio},
											journal={Microelectronic engineering},
											volume={4},
											number={3},
											pages={195--206},
											year={1986},
											publisher={Elsevier}
										}
										
										@article{gold_scattering_1988,
											title = {Scattering time and single-particle relaxation time in a disordered two-dimensional electron gas},
											volume = {38},
											issn = {0163-1829},
											url = {https://link.aps.org/doi/10.1103/PhysRevB.38.10798},
											doi = {10.1103/PhysRevB.38.10798},
											pages = {10798--10811},
											number = {15},
											journaltitle = {Physical Review B},
											author = {Gold, A.},
											urldate = {2020-04-20},
											date = {1988-11-15},
											langid = {english},
											file = {Gold - 1988 - Scattering time and single-particle relaxation tim.pdf:files/235/Gold - 1988 - Scattering time and single-particle relaxation tim.pdf:application/pdf}
										}
										
										@article{lee_low_1983,
											title = {Low field mobility of 2‐ \textit{d} electron gas in modulation doped Al $_{\textrm{ \textit{x} }}$ Ga $_{\textrm{ 1− \textit{x} }}$ As/{GaAs} layers},
											volume = {54},
											issn = {0021-8979, 1089-7550},
											url = {http://aip.scitation.org/doi/10.1063/1.331922},
											doi = {10.1063/1.331922},
											pages = {6432--6438},
											number = {11},
											journaltitle = {Journal of Applied Physics},
											author = {Lee, K. and Shur, M. S. and Drummond, T. J. and Morkoç, H.},
											urldate = {2020-04-20},
											date = {1983-11},
											langid = {english},
											file = {Lee et al. - 1983 - Low field mobility of 2‐ idi electron gas in .pdf:files/237/Lee et al. - 1983 - Low field mobility of 2‐ idi electron gas in .pdf:application/pdf}
										}
										
										

